On the Online Frank-Wolfe Algorithms for Convex and Non-convex Optimizations

In this paper, the online variants of the classical Frank-Wolfe algorithm are considered. We consider minimizing the regret with a stochastic cost. The online algorithms only require simple iterative updates and a non-adaptive step size rule, in contrast to the hybrid schemes commonly considered in the literature. Several new results are derived for convex and non-convex losses. With a strongly convex stochastic cost and when the optimal solution lies in the interior of the constraint set or the constraint set is a polytope, the regret bound and anytime optimality are shown to be ${\cal O}( \log^3 T / T )$ and ${\cal O}( \log^2 T / T)$, respectively, where $T$ is the number of rounds played. These results are based on an improved analysis on the stochastic Frank-Wolfe algorithms. Moreover, the online algorithms are shown to converge even when the loss is non-convex, i.e., the algorithms find a stationary point to the time-varying/stochastic loss at a rate of ${\cal O}(\sqrt{1/T})$. Numerical experiments on realistic data sets are presented to support our theoretical claims.

==> sections/online_app_nips.tex <==
\section{Online Learning Applications}
\label{sec:online}
We discuss several machine learning applications of the sFW and sAW algorithms. 
In the following, we show that \Cref{iii1} is satisfied with $\alpha = 0.5$ with $\noise_t = {\cal O}(\log t)$ in the examples below.
%Applying the sFW/sAW algorithms on these problems attain a learning rate of ${\cal O}(\log(t) / t)$ when the assumptions in \Cref{sec:main} are satisfied.  
The proofs on the corresponding convergence rates can be found in the supplementary materials. 
We summarize the learning rates in \Cref{tab:rate}. 
%A summary of the learning rates of the proposed online algorithms can be found below:

\begin{table}[t]
\caption{Learning rate of the sFW/sAW algorithms applied on different problems. Notice that we have only listed the dependence on iteration index $t$ and the dimensions of problems ($n$ for online SL and $m_1,m_2$ for online MC, see \Cref{sec:olasso} and \Cref{sec:omc}). All bounds are achievable with high probability. The sAW algorithm is not applicable for online MC as the constraint set is not atomic (\Cref{rem:atom}).} \label{tab:rate}
\begin{center} {\small
\begin{tabular}{| m{1.1cm} || c | c |} 
\hline
%Constants & $\noise_t$ & $\sigma$\\
& Online SL & Online MC \\
\hline 
sFW/sAW & $\displaystyle n \sqrt{ \frac{\log(nt)}{t} } $ & $\displaystyle  \sqrt{\frac{\log((m_1+m_2) t)}{t \cdot (m_1 \wedge m_2) / (m_1 \vee m_2)} } $ \tabularnewline 
\hline
sFW w/ \Cref{iii2},\Cref{iii3} & $\displaystyle  n^2  \frac{\log(nt)}{t} $  & $\displaystyle {\frac{\log((m_1+m_2) t)}{t  \cdot (m_1 \wedge m_2) / (m_1 \vee m_2)} }$ \tabularnewline 
\hline
sAW w/ \Cref{iii2} or \Cref{aw2} & $\displaystyle n^2  \frac{\log(nt)}{t}$ & Not Applicable \tabularnewline
\hline
\end{tabular}} \vspace{-.3cm}
\end{center}
\end{table}

\subsection{Online sparse learning} \label{sec:olasso} \vspace{-.1cm}
In the online sparse learning (SL) problem, we are sequentially 
given i.i.d.~observations $({\bm Y}_t, {\bm A}_t)$ such that ${\bm Y}_t \in \RR^m$ is
the response, ${\bm A}_t \in \RR^{m \times n}$ is the random design
and
\begin{equation} \label{eq:sparse_model}
{\bm Y}_t = {\bm A}_t \bar{\prm} + {\bm w}_t\eqs,
\end{equation}
where the vector ${\bm w}_t$ is i.i.d., $[{\bm w}_t]_i$ is independent of $[{\bm w}_t]_j$ for $i \neq j$ and $[{\bm w}_t]_i$ is zero-mean and sub-Gaussian with parameter $\sigma_w$. 
We suppose that the unkonwn parameter $\bar{\prm}$ is sparse. 
Attempting to learn $\bar{\prm}$, we solve the following optimization problem:
\begin{equation} \label{eq:olasso}
\min_{ \prm \in \RR^n } \Obj(\prm) \eqdef \frac{1}{2} \EE_{\bar{\prm}} [ \| {\bm Y}_t - {\bm A}_t \prm \|_2^2 ]~{\rm s.t.}~\| \prm \|_1 \leq r, 
\end{equation}
where $r > 0$ is a regularization constant. 

%${\bm A} \in \RR^{m \times n}$ is the feature vector/matrix that may be random. Furthermore, when conditioned on ${\bm A}$, the observation ${\bm Y} \in \RR^m$ is a random vector that is centered in ${\bm A} \bar{\prm}$, where $\bar{\prm}$ is unknown. This formulation is motivated by the scenario when $\bar{\prm}$ is sparse. 

%Our aim is to find the parameter $\prm^\star$ that minimizes \eqref{eq:olasso}. 
Similar setup has been studied in \cite{garrigues08,langford09}, which considered the case 
of  empirical squared loss, i.e., 
when $\Obj (\prm) = (1/2T) \sum_{s=1}^T \| {\bm Y}_s - {\bm A}_s \prm \|_2^2$ with $T \gg 1$. 

We propose the following online algorithm to \eqref{eq:olasso}. In the following, we initialize with the running estimates $\overline{(\bm{A}^\top \bm{Y})}_{0} = {\bm 0}$ and $\overline{(\bm{A}^\top \bm{A})}_{0} = {\bm 0}$. Consider the online implementations of sFW/sAW algorithm:

\noindent \textbf{Online SL Algorithm}. At time $t \geq 1$, we perform:
\begin{enumerate}
\item Select ${\bm A}_t$ and observe ${\bm Y}_t$ according to \eqref{eq:sparse_model}.
\item Evaluate the sufficient statistics:
\begin{equation*}
\begin{split}
\overline{(\bm{A}^\top \bm{Y})}_t & \eqdef (1 - t^{-1}) \overline{(\bm{A}^\top \bm{Y})}_{t-1} + t^{-1} {\bm A}_t^\top {\bm Y}_t, 
\\
\overline{(\bm{A}^\top \bm{A})}_t & \eqdef (1 - t^{-1}) \overline{(\bm{A}^\top \bm{A})}_{t-1} + t^{-1} {\bm A}_t^\top {\bm A}_t,
\end{split}
\end{equation*}
%where $\overline{(\bm{A}^\top \bm{Y})}_t$, $\overline{(\bm{A}^\top \bm{A})}_t$ are running 
and form the gradient estimate:
\begin{equation}\label{eq:grad_est_lasso}
\Hgrd \Obj_t (\prm) = \overline{(\bm{A}^\top \bm{A})}_t \prm - \overline{(\bm{A}^\top \bm{Y})}_t  \eqs.
\end{equation}
\item For sFW algorithm, proceed according to line~3 to line~4 in \Cref{alg:ofw}. For sAW algorithm, proceed according to line~3 to line~14 in \Cref{alg:ofw_away}. 
%Set $\atom_t = -r \cdot {\rm sign}([ \Hgrd \Obj_t (\prm_t) ]_i ) \cdot {\bm e}_i$, where $i = \arg \max_{j \in [n]} | [\Hgrd \Obj_t (\prm_t) ]_j |$, and ${\bm d}_t = {\bm a}_t + . 
%\item Update $\prm_{t+1} = (1- \gamma_t) \prm_t + \gamma_t \atom_t$, where $\gamma_t$ is defined in \Cref{alg:ofw}. 
\end{enumerate}
In the above, the linear optimization \eqref{eq:linear} or \eqref{eq:linear_away} can be evaluated as $\atom_t = -r \cdot {\rm sign}([ \Hgrd \Obj_t (\prm_t) ]_i ) \cdot {\bm e}_i$, where $i = \arg \max_{j \in [n]} | [\Hgrd \Obj_t (\prm_t) ]_j |$. We can derive:


% EXAMPLES to have online LASSO and REFERENCES

% A is a m \times n design matrix 

% A\prm + \epsilon_t, where the latter is that...

% FIXED design


% Use subgrassian




%Notice that:
%\begin{equation}
%\bm{\epsilon}_t = \Hgrd \Obj_t (\prm) - \grd \Obj (\prm) = - \frac{1}{tm} \sum_{s=1}^t {\bm A}^\top  {\bm w}_s \eqs
%\end{equation}
%is independent of $\prm$. 

% WRITE THE ACTUAL ALGORITHM
%Notice that \eqref{eq:grad_est_lasso} is an SA step for the stochastic gradient function. 

\begin{Prop} \label{prop:lasso}
Assume that $\| {\bm A}_t^\top {\bm A}_t -  \EE [{\bm A}^\top {\bm A}]  \|_{max} \leq B_1$ and $ \| {\bm A}_t \|_{max} \leq B_2$ almost surely, with $\| \cdot \|_{max}$ being the matrix max norm.
Define $\bm{\epsilon}_t (\prm) \eqdef \Hgrd \Obj_t (\prm) - \grd \Obj (\prm)$  and $c \eqdef \max_{ \prm \in \Cset } \| \prm - \bar{\prm} \|_1$.
With probability at least $1- (1+1/n)(\pi^2 \Delta / 6)$, the following holds for all $\prm \in \Cset$ and all $t \geq 1$:
\begin{equation} \label{eq:lassobd}
\| \bm{\epsilon}_t (\prm) \|_\infty \leq (c B_1 + \sqrt{m B_2\sigma_w^2}) \sqrt{ \frac{2 (\log(2n^2 t^2) - \log \Delta)}{t} } \eqs,
\end{equation}
where $\| \cdot \|_\infty$ is the infinity norm and the dual norm of $\| \cdot \|_1$.
\end{Prop}

%{ \color{red} verify H2, H3 and H4}
%
%\newpage
%Using triangular inequality, we can bound the gradient estimation error as:
%\begin{equation} \label{eq:ls1}
%\begin{array}{l}
%\displaystyle \| \bm{\epsilon}_t \|_\infty \leq \Big\| \frac{1}{t} \sum_{s=1}^t \big( {\bm A}_s^\top {\bm Y}_s - \EE [{\bm A}^\top {\bm Y}] \big) \Big\|_\infty \\
%\displaystyle ~~~~+ \Big\| \frac{1}{t} \sum_{s=1}^t \big( {\bm A}_{s}^\top {\bm A}_{s} - \EE [{\bm A}^\top {\bm A}]  \big) \prm \Big\|_\infty 
%\end{array} 
%\end{equation}
%To bound the second term in \eqref{eq:ls1}, we define ${\bm Z}_s \eqdef {\bm A}_{s}^\top {\bm A}_{s} - \EE [{\bm A}^\top {\bm A}] $. Observe that
%\begin{equation}
%\Big\| \frac{1}{t} \sum_{s=1}^t {\bm Z}_s  \prm \Big\|_\infty = \max_{i \in [n]} \Big| \frac{1}{t} \sum_{s=1}^t {\bm z}_{s,i} \prm \Big|,
%\end{equation}
%where $ {\bm z}_{s,i}$ denotes the $i$th row vector in ${\bm Z}_s$. Furthermore, by the Holder's inequality,
%\[
%\big| \frac{1}{t} \sum_{s=1}^t {\bm z}_{s,i} \prm \big| \leq \| \prm \|_1 \cdot \big\| \frac{1}{t} \sum_{s=1}^t {\bm z}_{s,i} \big\|_\infty,
%\]
%Now that ${\bm z}_{s,i}$ is a zero-mean, independent random vector with elements bounded in $[-B_1,B_1]$, applying the union bound and the Hoefding's inequality gives:
%\begin{equation} \label{eq:ls2}
%\PP \big( \big\|\textstyle  (1/t) \sum_{s=1}^t {\bm z}_{s,i} \big\|_\infty \geq \delta,~\forall~i \big) \leq 2n^2 \rme^{-\frac{\delta^2 t}{2B_1^2}}.
%\end{equation}
%Setting $\delta = B_1 \sqrt{2 (\log(2n^2 t^2) - \log \Delta) / t}$ gives $\Delta / t^2$ on the right hand side. With probability at least $1 - \Delta / t^2$, we have 
%\begin{equation} \label{eq:lsbound}
%\Big\| \frac{1}{t} \sum_{s=1}^t {\bm Z}_s \prm \Big\|_\infty \leq r B_1 \sqrt{2 (\log(2n^2 t^2) - \log \Delta) / t},
%\end{equation}
%
%%which can be upper bounded as:
%%\begin{equation}
%%\| \bm{\epsilon}_t \|_\infty \leq \| {\bm A} \|_{\sigma, \infty}  \Big\| \frac{1}{t} \sum_{s=1}^t \big( \EE [{\bm y}_{i(s)}] - {\bm y}_{i(s)} \big) \Big\|_\infty.
%%\end{equation}
%To bound the first term in \eqref{eq:ls1}, we observe that ${\bm A}_s^\top {\bm Y}_s - \EE [{\bm A}^\top {\bm Y}]$ is again a zero-mean, independent vector with elements bounded in $[-B_2,B_2]$, similarly we can apply the Hoefding's inequality:
%\begin{equation} \label{eq:ls3}
%\PP \Big( \Big\| \frac{1}{t} \sum_{s=1}^t {\bm A}_s^\top {\bm Y}_s - \EE [{\bm A}^\top {\bm Y}] \Big\|_\infty  \geq \delta \Big) \leq 2n \rme^{-\frac{\delta^2 t}{2 B_2^2}}.
%\end{equation}
%Setting $\delta = B_2 \sqrt{2 (\log(2n^2 t^2) - \log \Delta) / t}$ gives $\Delta / (nt^2)$ on the right hand side. 
%Finally, combining the above result with \eqref{eq:lsbound} and using a union bound argument for all $t \geq 1$ yield \eqref{eq:largescale}. 
%\hfill \textbf{Q.E.D.}


We observe that \Cref{iii1} is satisfied with $\noise_t$ asymptotically equivalent to $4 {\log (t) }$ and $\alpha = 0.5$. 
Furthermore, \Cref{iii0} is satisfied if $M {\bf I} \succeq \EE [ {\bm A}^\top {\bm A} ]$; \Cref{iii2} is satisfied if $\EE [ {\bm A}^\top {\bm A} ] \succeq \mu {\bf 1}$ for some $\mu > 0$; and \Cref{aw1} is satisfied as $\Cset$ is a polytope. 
%with $\bar{\Delta} = (1+1/n) (\pi^2 \Delta / 6)$, $\sigma = (c B_1 + \sqrt{m B_2\sigma_w^2}) \sqrt{2}$ and $\noise_t = \log(2n^2t^2) - \log \Delta$. 
The convergence analysis from the previous section applies. The learning rates can be found in \Cref{tab:rate}. 

\begin{Remark}
\cite{langford09} has applied a stochastic proximal gradient  (sPG) method to solve an $\ell_1$ regularized variant of \eqref{eq:olasso} for empirical risk minimization. From their result, if the number of iterations run $T$ is known a-priori, then the convergence rate is ${\cal O}(1/\sqrt{T})$. This is similar to the sFW algorithm, yet the sFW algorithm has a better sparsity-accuracy tradeoff; see \cite{Jaggi13}. 
%Previous works \cite{} have applied variants of stochastic projected gradient (SPG) method to solve \eqref{eq:olasso}, where a convergence rate of ${\cal O}(??)$ is provided. The rate is similar to the sFW algorithm. The per-iteration complexity of SPG is ${\cal O}(n \log n)$ as the projection step involves sorting $\prm_t$ \cite{}. In comparison, the per-iteration complexity of sFW is only ${\cal O}(n)$. % some convergence rate....
\end{Remark}




% COMPARISON TO PROJECTED GRADIENT ALGORITHM 



\subsection{Online Matrix Completion} \label{sec:omc}
%We cast the online matrix completion task in the so-called \emph{transductive} model \cite{}. 
We consider the matrix completion problem
when the observation distribution belongs to the natural exponential
family. This distribution family is general enough to encompass
many distributions encountered in practice. For example,
Gaussian matrix completion can be used for recommender systems
\cite{Candes_Plan10,Negahban_Wainwright12,Klopp14}, Poisson matrix completion 
for image recovery \cite{Cao_Xie15} and logistic for one-bit completion 
\cite{Davenport_Plan_VandenBerg_Wootters12}.
%Say that Exp family covers distritubion used in parctice
%that 
We are sequentially  given \iid~
 observations   
in the form $(k_{t},l_{t},\Y_{t})$, with $(k_{t}, l_{t}) \in [m_1]\times [m_2]$ 
and $\Y_{t} \in \RR$. The conditional
distribution  of $\Y_{t}$ \wrt the sampling
is parametrized by
an unknown matrix $\tX \in \matset{m_1}{m_2}$
and supposed to belong to the exponential family.
More precisely, the conditional density 
of $\Y_t$ is given by
\begin{equation} \label{eq:y_dist}
p_{\tX}(\Y_t | k_t, l_t ) \eqdef
%\Exp{\bms}{\lgp}{\tX_{k_s,l_s}}(\Y_s) 
 \bms(\Y_{t}) \exp\left(\Y_{t} \tX_{k_{t},l_{t}} - \lgp(\tX_{k_{t},l_{t}}) \right) \eqs,  
\end{equation}
where $\bms(\cdot)$ and $\lgp(\cdot)$ are the base measure and log-partition functions,
respectively.
% It can be shown (\eg \cite[Proposition 3.1]{Wainwright_Jordan08}), that the 
% log-partition function $\lgp (\cdot)$
% is convex and admits derivatives of all orders on its domain.

For any $\prm \in \matset{m_1}{m_2}$,
the Kullback-Leibler divergence between the 
distribution associated with $\prm$ and the
true distribution with $\bar{\prm}$ is (up to an additive constant):
\begin{equation}
\label{def:bregman}
\Obj(\prm) \eqdef  \EE_{\bar{\prm}} \big[  \lgp(\prm_{k_{1},l_{1}})- \Y_{1} \prm_{k_{1},l_{1}}
%- \log(\bms(Y_{t,i}))
\big] 
\eqs.
\end{equation}
Note that in the example of Gaussian noise,
$\Obj(\cdot)$ is simply the square loss function.
We are interested in minimizing 
the Kullback-Leibler divergence \eqref{def:bregman}
under a penalty favoring low rank solutions.
In the following we consider a trace norm 
penalty $\|\cdot\|_{\sigma,1}$ defined as the
sum of the singular values.
In such case the problem boils down to
% the  
%trace norm constrained problem:
\begin{equation} 
\label{eq:min_pb}
\min_{ \prm \in \contset_\trad} \Obj(\prm) \quad \text{with} \quad
\Cset_\trad \eqdef \{ \prm  : \|\prm\|_{\sigma,1}
\leq \trad  \} \eqs,
\end{equation}

% 
% Online matrix completion problems have recently been considered in an empirical 
% risk minimization setting. In contrast,
% we focus on a probabilistic observation setting to minimize the expected risk. 

We propose the following online implementation of the sFW algorithm to \eqref{eq:min_pb}:

\noindent \textbf{Online MC Algorithm}. At time $t \geq 1$, we perform:
\begin{enumerate}
\item Receive a new observation $(k_t,l_t,{\Y}_{t})$ 
and update the sufficient statistics as follows:
\begin{align*}
&S^{(1)}_t = (1-t^{-1}) S_{t-1}^{(1)} + t^{-1} \Y_t e_{k_{t}} e^{'\top}_{l_{t}}\\
&S^{(2)}_t = (1-t^{-1}) S_{t-1}^{(2)} + t^{-1}   e_{k_{t}} e^{'\top}_{l_{t}}
\end{align*}
with $(e_k)_{k=1}^{m_1}$ (\resp $(e'_l)_{l=1}^{m_2}$) the canonical basis of
of $\RR^{m_1}$ (\resp $\RR^{m_2}$).
%\begin{equation}
%\Y_t | (k_t,l_t) \sim 
%%\Exp{\bms}{\lgp}{\tX_{k_s,l_s}}(\Y_s) 
% \bms(\Y_t) \exp\left(\Y_t \tX_{k_t,l_t} - \lgp(\tX_{k_t,l_t}) \right)  \eqs,
%\end{equation}
\item Evaluate the gradient estimate as:
\begin{align*}
& [\Hgrd \Obj_t (\prm)]_{k,l} = \lgp'(\prm_{k,l})[S^{(2)}_t]_{k,l} - [S^{(1)}_t]_{k,l}\eqs,
\end{align*}
for all $k,l \in [m_1] \times [m_2]$.
\item Set $\atom_t = - \trad {\bm u}_1 {\bm v}_1^\top$, 
where ${\bm u}_1,{\bm v}_1$ are the top singular vectors of $\Hgrd \Obj_t (\prm_t)$. 
\item Update $\prm_{t+1} = (1-\gamma_t) \prm_t + \gamma_t \atom_t$.
\end{enumerate}


% In this setting, the exhaustive statistic is given by:
% \begin{equation*}
%   \exs_t \eqdef \frac{1}{t} \sum_{s=1}^t \Y_t e_{k_t} e'^\top_{l_t}
% \end{equation*}
% with $(e_k)_{k=1}^{m_1}$ (\resp $(e'_l)_{l=1}^{m_2}$) the canonical basis of
% of $\RR^{m_1}$ (\resp $\RR^{m_2}$). Similar to the case of online LASSO, a straightforward approximation of the gradient could be
% $
% \lgpm'( \prm) - \exs_t,
% $
% with $ (\lgpm'(\prm))_{k,l} \eqdef (m_1m_2)^{-1}\lgp(\prm_{k,l})$ for any $k,l \in [m_1] \times [m_2]$.
% However, when $m_1m_2 \gg 1$ holds, computing $\lgpm'(\prm)$ is expensive. 

%Given a 
%matrix $\prm$,
%the objective gradient can be approximated by the following quantity:
%\begin{equation*}
%  \Hgrd \Obj_t (\prm) =\frac{1}{t} \sum_{s=1}^t \left( \lgp'(\prm_{k_s,l_s}) - \Y_s \right)  e_{k_s} e^{'\top}_{l_s} \eqs,
%\end{equation*}
%with $(e_k)_{k=1}^{m_1}$ (\resp $(e'_l)_{l=1}^{m_2}$) the canonical basis of
%of $\RR^{m_1}$ (\resp $\RR^{m_2}$).

%OTHER COUNTER FOR ASSULOTIONS
In order to control the gradient estimation error,
we assume the following on the noise.
\begin{assumptionb}
\label{A1}
The noise variance is finite, that is
there exists a constant
$\sigup >0$ such that for all $\vartheta \in \RR$,
$
0 \leq \lgp''(\vartheta)  \leq \sigup^2  \eqsp,
$
and the noise is sub-exponential \ie
there exist a constant $\sexp \geq 1$ such 
that for all $(k,l) \in [m_1] \times [m_2]$:
\begin{equation}
\label{eq:def_sub}
\int\exp\left(\lambda^{-1}\left|y - \lgp'(\tX_{k,l})\right|\right)p_{\tX}(y|k,l)dy \leq \rme \eqs,
\end{equation}
where $p_{\tX}(\cdot)$
is define in \eqref{eq:y_dist} and
$\rme$ is the natural number.
\end{assumptionb}
\begin{assumptionb}
\label{A2}
There exists a finite constant $\mrc>0$
such that for all $\prm \in \contset$, $k \in [m_1]$, $l \in [m_2]$
\begin{equation}
 \mrc \geq \max
 \left( \sqrt{\sum_{l=1}^{m_2} \lgp'(\prm_{k,l})^2},
 \sqrt{\sum_{k=1}^{m_1} \lgp'(\prm_{k,l})^2} \right) \eqs.
\end{equation}

Notice that $\mrc = {\cal O}( \sqrt{ \max\{ m_1, m_2 \} } )$.

\end{assumptionb}
We remark that \Cref{A1} and \Cref{A2} are satisfied by all the
above mentioned exponential family distributions.
Define $d \eqdef m_1 + m_2$, 
%then with these assumptions and notation, 
the approximation error can be controlled as follows.
\begin{Prop} 
\label{prop:gradient_conc}
Assume \Cref{A1}, \Cref{A2}
and that the sampling distribution is uniform.
% and
%define
%$\bm{\epsilon}_t (\prm) \eqdef $.
Define
the approximation error
$\bm{\epsilon}_t (\prm) \eqdef \Hgrd \Obj_t( \prm ) - \nabla f(\prm)$.
With probability at least $1-  \Delta$, 
for any 
$t \geq T_\Delta \eqdef  (\sexp/\sigup)^2 \log^2(\sexp/\sigup)\log(d+2d/\Delta)$,
and any $\prm \in \contset_\trad$:
\begin{equation*}
\label{eq:grad_dev} 
 \normop{\bm{\epsilon}_t (\prm)} = \mathcal{O} \left( c_{\sexp } \left( \mrc 
  + \sigup  \right) 
  \sqrt{ \frac{\log(d(1 + t^2 /\Delta)) }{t(m_1 \wedge  m_2)}} \right) \eqs,
\end{equation*}
with
$\|\cdot\|_{\sigma, \infty}$ the 
operator norm, $c_\sexp$ a constant which depends only on $\sexp$. The constants $\sexp$, $\sigup$ and $\mrc$ are 
defined in \Cref{A1} and \Cref{A2}.
\end{Prop}
\begin{Remark}
Vectorizing the  matrix completion problem
and applying the same analysis as for the 
online sparse learning would yield a
dimension dependency of 
$\sqrt{m_1m_2}$. However, taking into account the
nature of the problem drastically reduces it to 
$\mathcal{O}(\sqrt{(m_1 \vee  m_2) / (m_1 \wedge  m_2)})$.
\end{Remark}
In light of \Cref{prop:gradient_conc}, 
\Cref{iii1} is satisfied  for $\noise_t \propto \log(t)$
and $\alpha = 0.5$. Besides, from \Cref{A1},
\Cref{iii0} is satisfied for $\Curve = \sigup$.
the results from \Cref{thm:converge} applies.
Moreover, \Cref{iii2} is satisfied if 
$\lgp''(\vartheta) \geq \mu$ for some $\mu >0$ 
and $\vartheta \in \Cset$. Therefore the previous
analysis on sFW applies to the online matrix completion problem.


